Hardness Amplification for (Sparse) LPN

We prove new hardness amplification results for Learning Parity with Noise ($\mathsf{LPN}$) and its sparse variants. In $\mathsf{LPN}_{\eta,n,m}$, the goal is to recover a secret $\vec s\in\mathbb{F}_2^n$ from $m$ noisy linear samples $(\vec a,b)$, where $\vec a\leftarrow \mathbb{F}_2^n$ is uniform and $b=\langle \vec a,\vec s\rangle + e$ with $e\leftarrow \mathrm{Ber}(\eta)$. Building on the direct-product framework introduced by Hirahara and Shimizu [HS23], we show an 'instance-fraction amplification' theorem: for any $\varepsilon,\delta>0$, any algorithm that solves $\mathsf{LPN}_{\eta,n,m}$ with success probability $\varepsilon$ can be transformed into an algorithm that succeeds with probability $1-\delta$ on a related $\mathsf{LPN}$ distribution with scaled parameters $\mathsf{LPN}_{\eta/k,\;n/k,\;m}$, where $ k=\Theta\!\left(\frac{1}{\delta}\log\frac{1}{\varepsilon}\right). $ Equivalently, an algorithm that solves $\mathsf{LPN}$ on a 'small fraction of instances' can be converted into an algorithm that solves $\mathsf{LPN}$ on 'almost all instances', yielding a self-amplification for a wide range of parameters. We extend the same amplification approach to $\mathsf{LPN}$ over $\mathbb{F}_q$ and to Sparse-$\mathsf{LPN}$, where each query vector $\vec a$ has exactly $\sigma$ nonzero entries. Together, these results establish hardness self-amplification for a broad family of $\mathsf{LPN}$-type problems, strengthening the foundations for assuming the average-case hardness of $\mathsf{LPN}$ and its sparse variants.

==> reduction_for_sparse_case.tex <==

    
In this section we will give a reduction from $\lpn^{\approx s}_{\varepsilon,n,q}$ to $\lpn^{= 2s}_{\varepsilon,2n,q}$. Our approach will be as follows, given an instance $(\vec A, \vec b= \vec A \cdot \vec s+ \vec e)$ of $\lpn_{\eta,n,q}^{\approx s}$, we will output $\mathcal{R}\paren{\vec A, \vec b}=\paren{\vec A', \vec b '}$, such that distribution of $\paren{\vec A', \vec b'}$ is statistically close to the distribution induced by an instance of $\lpn_{\eta,2n,q}^{=2s}$. We also need the secret $\vec s$ for the original $\lpn_{\eta,n,q}^{\approx s}$ instance, to be easily computable given the secret $\vec s'$ of $(\vec A', \vec b')$. Now, if an algorithm $\mathcal{A}$ can solve $\lpn_{\eta,2n,q}^{=2s}$ with success probability $\alpha$ then given the above reduction it can solve $\lpn_{\eta,n,q}$ with success probability $\alpha - \delta$, where $\delta $ is the distance between the distribution induced by the reduction, and the distribution induced by $\lpn_{\eta,2n,q}^{=2s}$.
\subsection{Details of the Reduction
}
Given an instance of $\lpn_{\eta,n,q}^{\approx s}$ as,


$$\paren{\vec A = \begin{bmatrix}
\vec a_1 \\
\vec a_2 \\
\vdots \\
\vec a_q
\end{bmatrix}, ~ \vec b=\begin{bmatrix}
b_1 \\
b_2 \\
\vdots \\
b_q
\end{bmatrix}
  },$$
we will check if for all $i\in [q]$, $\norm{\vec a _i}_0\leq 2s$, otherwise we will output $\perp$. Assuming the above condition holds, for all $i \in [q]$ we define $t_i= 2s-\norm{\vec a_i}_0$ and sample $\vec a_i^{*} \sim {[n] \choose 2s-t_i}$, uniformly. 
We also sample a $\vec s ^{*} \sim \F_2^{n}$, uniformly and finally output $\mathcal{R}(\vec A, \vec b)$ as,
\[
\paren{\vec A' = \begin{bmatrix}
\vec a_1 || \vec a^{*}_1 \\
\vec a_2 || \vec a^{*}_2\\
\vdots \\
\vec a_q || \vec a^{*}_q
\end{bmatrix}, ~ \vec b'=\begin{bmatrix}
b_1 +\langle\vec a^{*}_1 , \vec s^{*} \rangle\\
b_2 +\langle\vec a^{*}_2 , \vec s^{*} \rangle\\
\vdots \\
b_q +\langle\vec a^{*}_q , \vec s^{*} \rangle
\end{bmatrix}
  },
\]
 We will now prove the distribution of $(\vec A', \vec b')$ is statistically close to the distribution of the instances of $\lpn_{\eta,2n,q}^{= 2s}$.



\subsection{Proof of Working}
We will first prove the following lemma which claims that each row of $\vec A'$ is statistically close to the uniform distribution over ${[2n] \choose 2s}$,
\begin{lemma}
    Consider the following distributions over ${[2n] \choose 2s} \cup \{\perp\}$,
    \begin{enumerate}
        \item $\mathcal{D}_1$- This is the uniform distribution over ${2n \choose 2s}$,\[
\Pr_{\mathbf{S}\sim \mathcal{D}_1}[\mathbf{S}=T]
=
\begin{cases}
\displaystyle \binom{2n}{2s}^{-1}, & \text{if } T\in \binom{[2n]}{2s},\\[6pt]
0, & \text{if } T=\perp.
\end{cases}
\]

        \item $\mathcal{D}_2$- For sampling from $\mathcal{D}_2$, we first sample $\vec a$ from $\paren{\text{Ber}(s/n)}^n$. Now if $\norm{\vec a}_0 >2s$ we output $\perp$, otherwise we sample $\vec a^* \sim {[n] \choose 2s-\norm{\vec a}_0}$ and output $\paren{\vec a || \vec a ^*}$. 
  \[
\Pr_{\mathbf{S}\sim \mathcal{D}_2}[\mathbf{S} = T]
=
\begin{cases}
\displaystyle 
\binom{n}{\,2s-t\,}^{-1} 
\left(1-\tfrac{s}{n}\right)^{\,n-t}
\left(\tfrac{s}{n}\right)^{t}, 
& \quad \text{if } T = (\vec{a}, \vec{a}^*) \in \tbinom{[2n]}{2s}
  \text{ and } \norm{\vec{a}}_0 = t, \\[10pt]
\displaystyle 
\sum_{i=2s+1}^{n} \binom{n}{i} 
\left(1-\tfrac{s}{n}\right)^{\,n-i}
\left(\tfrac{s}{n}\right)^{i}, 
& \quad \text{if } T = \perp.
\end{cases}
\]

    \end{enumerate}
    Then for sufficiently large $n$, it holds that ,
    \[\Delta \paren{\mathcal{D}_1,\mathcal{D}_2} \leq \operatorname{negl}(n).\]
\end{lemma}

   By the definition of statistical distance, we know that,
\[
\begin{aligned}
\Delta\!\left(\mathcal{D}_1, \mathcal{D}_2\right)
&= \tfrac{1}{2} \sum_{T} \bigl| \mu_{\mathcal{D}_1}(T) - \mu_{\mathcal{D}_2}(T) \bigr|\\
&= \sum_{\substack{T : \mu_{\mathcal{D}_1}(T) \geq \mu_{\mathcal{D}_2}(T)}} 
    \bigl( \mu_{\mathcal{D}_1}(T) - \mu_{\mathcal{D}_2}(T) \bigr)\leq\sum_{\substack{T : \mu_{\mathcal{D}_1}(T) \geq \mu_{\mathcal{D}_2}(T)}} 
     \mu_{\mathcal{D}_1}(T),\\
&= \sum_{\substack{T : \mu_{\mathcal{D}_2}(T) \geq \mu_{\mathcal{D}_1}(T)}} 
    \bigl( \mu_{\mathcal{D}_2}(T) - \mu_{\mathcal{D}_1}(T) \bigr)\leq \sum_{\substack{T : \mu_{\mathcal{D}_2}(T) \geq \mu_{\mathcal{D}_1}(T)}} 
     \mu_{\mathcal{D}_2}(T).
\end{aligned}
\]
Hence, to give an upper bound on the statistical distance of the two distributions we will identify the $T$'s for which $\mu_{\mathcal{D}_1}(T)> \mu_{\mathcal{D}_2} (T)$. Then we will give an upper bound on $\sum_{\substack{T : \mu_{\mathcal{D}_2}(T) \geq \mu_{\mathcal{D}_1}(T)}} 
     \mu_{\mathcal{D}_2}(T)$, for giving an upper bound to $\Delta\paren{\mathcal{D}_1,\mathcal{D}_2}$. We will use the following lemma in order to identify when is $\mu_{\mathcal{D}_1}(T)> \mu_{\mathcal{D}_2} (T)$,

\begin{lemma}
    For sufficiently large $n$, $s=\mathcal{O}(\log n)$. For $t \in [0.99s, 1.01 s]$ we have that,

\[\left(1-\tfrac{s}{n}\right)^{\,n-t}
\left(\tfrac{s}{n}\right)^{t} < \dfrac{\binom{n}{\,2s-t\,}}{\binom{2n}{2s}}. \]
\end{lemma}
\begin{proof}
   Let 
\[
p(t) = \left(1-\tfrac{s}{n}\right)^{\,n-t}
        \left(\tfrac{s}{n}\right)^{t},
\qquad
q(t) = \dfrac{\binom{n}{\,2s-t\,}}{\binom{2n}{2s}}.
\]
From this we have,
\begin{align*}
    \dfrac{q(t)}{p(t)}
    &= \dfrac{\dfrac{n!\,(2s)!\,(2n-2s)!}{(2s-t)!\,(n-2s+t)!\,(2n)!}}
            {\left(\tfrac{n-s}{n}\right)^{\,n-t}
             \left(\tfrac{s}{n}\right)^{t}}, \\[12pt]
    &= \dfrac{n!\,(2s)!\,(2n-2s)!}
            {(2s-t)!\,(n-2s+t)!\,(2n)!}
       \cdot
       \left(\tfrac{n}{\,n-s}\right)^{n-t}
       \cdot
       \left(\tfrac{n}{s}\right)^{t},\\[12pt]      &\;\approx\;
\sqrt{ \frac{ s(2n-2s) }{ (2s-t)\,\bigl(n-2s+t\bigr) } }
\cdot
\dfrac{ n^n \,(2s)^{2s}\,(2n-2s)^{2n-2s} }
      { (2s-t)^{2s-t}\,\bigl(n-2s+t\bigr)^{\,n-2s+t}\,(2n)^{2n} }
\cdot
\left(\tfrac{n}{\,n-s}\right)^{n-t}
\left(\tfrac{n}{s}\right)^{t},\\[12pt]
&=\sqrt{ \frac{ s(2n-2s) }{ (2s-t)\,\bigl(n-2s+t\bigr) } }
\cdot\paren{\dfrac{s}{2s-t}}^{(2s-t)}\cdot \paren{\dfrac{n-s}{n-2s+t}}^{n-2s+t},
\\[12pt]
&=\sqrt{ \frac{ s(2n-2s) }{ (2s-t)\,\bigl(n-2s+t\bigr) } }
\cdot\paren{\dfrac{s}{2s-t}}^{(2s-t)}\cdot \paren{1+\dfrac{s-t}{n-2s+t}}^{n-2s+t}.\\
\end{align*}
Note that $\sqrt{ \frac{ s(2n-2s) }{ (2s-t)\,\bigl(n-2s+t\bigr) } }$ is always greater than $1$, because for sufficiently large $n$,
\begin{align*}
    s(2n-2s)-(2s-t)(n-2s+t)=nt +2s^2-4st>0\\
\end{align*}
When $t \in [0.9s,s)$, then $\paren{\dfrac{s}{2s-t}}\geq \frac{10}{11}$. Using Taylor's theorem we get that for sufficiently large $x$, $(1+\frac{1}{x})^x>e \cdot e^{-\frac{1}{2x}}$. Which gives us for sufficiently large $n$,
\[
\dfrac{q(t)}{p(t)}> \paren{\frac{10}{11}}^{s-t}\cdot e^{(s-t)} \cdot e^{-\paren{\frac{s-t}{2n-4s+2t}}}>1.
\]
When $t=s$ we get,
\[\dfrac{q(t)}{p(t)}\geq \sqrt{ \frac{ s(2n-2s) }{ (2s-t)\,\bigl(n-2s+t\bigr) } }>1.
\]
When $t \in (s,1.01s]$, if we take $(1-\frac{t}{s})=x$, then,
\[\dfrac{q(t)}{p(t)} \approx \paren{\dfrac{1}{1-x}}^{(1-x)s} \cdot e^{-xs} \cdot e^{\paren{\frac{t-s}{2n-4s+2t}}}\] \rnote{The proof breaks down here cause $(1/1-x)^{(1-x)} < e$ near x=0 )}
\qed\end{proof}
